Gas cooling of test masses for future gravitational-wave observatories

Recent observations made with Advanced LIGO and Advanced Virgo have initiated the era of gravitational-wave astronomy. The number of events detected by these "2nd Generation" (2G) ground-based observatories is partially limited by noise arising from temperature-induced position fluctuations of the test mass mirror surfaces used for probing spacetime dynamics. The design of next-generation gravitational-wave observatories addresses this limitation by using cryogenically cooled test masses; current approaches for continuously removing heat (resulting from absorbed laser light) rely on heat extraction via black-body radiation or conduction through suspension fibres. As a complementing approach for extracting heat during observational runs, we investigate cooling via helium gas impinging on the test mass in free molecular flow. We establish a relation between cooling power and corresponding displacement noise, based on analytical models, which we compare to numerical simulations. Applying this theoretical framework with regard to the conceptual design of the Einstein Telescope (ET), we find a cooling power of 10 mW at 18 K for a gas pressure that exceeds the ET design strain noise goal by at most a factor of $\sim 3$ in the signal frequency band from 3 to 11 Hz. A cooling power of 100 mW at 18 K corresponds to a gas pressure that exceeds the ET design strain noise goal by at most a factor of $\sim 11$ in the band from 1 to 28 Hz.

==> text/systematic_uncertainties.tex <==
\section{\textcolor{red}{Systematic uncertainties}}
\label{sec:systematic-uncertainties}
In our modelling approach, we assume unity accommodation for both transfer of heat and tangential momentum between helium atoms and surfaces of TM and frame (see~\autoref{sec:suspended-mirror-setup}).
We settled on this approach, as we did not find corresponding values for the interaction between helium and silicon, at the discussed temperatures, in literature. 
Reference~\cite{corruccini1959gaseous} suggests to use values of 0.6 (1) for the thermal accommodation coefficient $\alpha_\mathrm{T}$ of helium for \SI{20}{K} (\SI{4}{K}), based on measurements with glass and metal surfaces. 
For the tangential momentum accommodation coefficient $\alpha_\mathrm{M}$, Ref.~\cite{agrawal2008survey} reports for silicon at room temperature a value of 0.923, as a mean value of different measurements reported in literature. 
\cite{cao2005temperature} presents a model, which predicts that $\alpha_\mathrm{M}$ increases for decreasing temperature.

Our assumption of unity accommodation for heat transfer at the frame and for tangential momentum at frame and TM appears to be consistent with the previous considerations.
Note that $\alpha_\mathrm{M}=1$ corresponds to the worst case.
The assumption of unity accommodation for heat transfer at the TM, however, might be optimistic. 
The assumption of $\alpha_\mathrm{T}=0.6$ for the TM corresponds to a 40~\% reduction in cooling power (i.e., $P_\mathrm{gas}\rightarrow\alpha_\mathrm{T}P_\mathrm{gas}$ in~\autoref{eq:cooling_power2} and~\ref{eq:cooling_T_scaling}).
This relies on the assumption that the gas outgoing from the TM has a Maxwellian velocity distribution.
As a consequence of this partial accommodation, TMs need to be heavier by $\sim30~\%$ (i.e., $m_\mathrm{TM}=387~\mathrm{kg}$), for similar values of cooling power and noise as reported in Sec.~\ref{sec:cooling-power-and-added-thermal-noise-for-et-design}. 
